Revisiting Zeroth-Order Optimization for Memory-Efficient LLM Fine-Tuning: A Benchmark

In the evolving landscape of natural language processing (NLP), fine-tuning pre-trained Large Language Models (LLMs) with first-order (FO) optimizers like SGD and Adam has become standard. Yet, as LLMs grow {in size}, the substantial memory overhead from back-propagation (BP) for FO gradient computation presents a significant challenge. Addressing this issue is crucial, especially for applications like on-device training where memory efficiency is paramount. This paper proposes a shift towards BP-free, zeroth-order (ZO) optimization as a solution for reducing memory costs during LLM fine-tuning, building on the initial concept introduced by MeZO. Unlike traditional ZO-SGD methods, our work expands the exploration to a wider array of ZO optimization techniques, through a comprehensive, first-of-its-kind benchmarking study across five LLM families (Roberta, OPT, LLaMA, Vicuna, Mistral), three task complexities, and five fine-tuning schemes. Our study unveils previously overlooked optimization principles, highlighting the importance of task alignment, the role of the forward gradient method, and the balance between algorithm complexity and fine-tuning performance. We further introduce novel enhancements to ZO optimization, including block-wise descent, hybrid training, and gradient sparsity. Our study offers a promising direction for achieving further memory-efficient LLM fine-tuning. Codes to reproduce all our experiments are at https://github.com/ZO-Bench/ZO-LLM .

==> tables/accuracy.tex <==
\begin{table}[htb]
    \centering
    \caption{Test accuracy ranking of different methods measured across tasks for OPT 13B model. It is measured on 80GB A100s with PCIe connections. }
    \label{tab: accuracy}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcc|lcc}
    \toprule[1pt]
    \midrule
    \multicolumn{3}{c}{Memory Ranking} & \multicolumn{3}{|c}{Wall-Clock Time Ranking} \\
    \midrule
    Optimizer    & Hardware          & Memory $\Downarrow$ & Optimizer    & Hardware          & Step Time $\Downarrow$ \\
    \midrule
    ZO-SGD       & 1xA100  & $51$ GB             & FO-SGD       & 2xA100 & 1.88 s        \\
    ZO-SGD-Cons  & 1xA100  & $51$ GB             & FO-Adam      & 3xA100 & 1.96 s        \\
    ZO-SGD-Sign  & 1xA100  & $51$ GB             & ZO-SGD-MMT   & 2xA100 & 2.00 s        \\
    FO-SGD       & 2xA100 & $101$ GB            & ZO-Adam      & 3xA100 & 2.15 s        \\
    ZO-SGD-MMT   & 2xA100 & $104$ GB            & Forward-Grad & 2xA100 & 2.29 s        \\
    Forward-Grad & 2xA100 & $105$ GB            & ZO-SGD-Sign  & 1xA100  & 2.38 s        \\
    ZO-Adam      & 3xA100 & $158$ GB            & ZO-SGD       & 1xA100  & 2.39 s        \\
    FO-Adam      & 3xA100 & $231$ GB            & ZO-SGD-Cons  & 1xA100  & 4.92 s \\
    \midrule
    \bottomrule[1pt]
    \end{tabular}
    }
    \vspace*{-2em}
\end{table}




==> tables/main_results.tex <==
\begin{table}[htb]
\centering
\caption{}
\label{tab: result_main}
\resizebox{.7\linewidth}{!}{%
\begin{tabular}{lcccc}
\toprule[1pt]
\midrule
\multicolumn{1}{c}{} & \textbf{FT}   & \textbf{LoRA} & \textbf{Prefix} & \textbf{Prompt} \\
\midrule
\multicolumn{5}{c}{\texttt{OPT-1.3B}, SST2}                   \\
\midrule
FO-SGD               & 91.1 & 93.6 & 93.1   & 92.8   \\
FO-Adam              & 90.1 & 93.7 & 93.9   & 91.7   \\
\midrule
ZO-SGD               & 89.9 & 90.1 & 91.4   & 84.4   \\
ZO-SGD-MMT           & 85.2 & 91.3 & 91.2   & 86.9   \\
ZO-SGD-CONS          & 88.3 & 90.5 & 81.8   & 84.7   \\
ZO-Sign-SGD          & 87.2 & 91.5 & 89.5   & 72.9   \\
ZO-Adam              & 84.4 & 92.3 & 91.4   & 75.7   \\
Forward-Grad         & 90.3 & 90.3 & 90.0   & 82.4  \\
\midrule
\multicolumn{5}{c}{\texttt{OPT-13B}, COPA}
\\
\midrule
FO-SGD               & 86 & 88   & 80     & 89     \\
FO-Adam              & 90 & 88   & 88     & 85     \\
\midrule
ZO-SGD               & 90 & 87   & 79     & 80     \\
ZO-SGD-MMT           & 87 & 84   & 85     & 84     \\
ZO-SGD-CONS          & 82 & 88   & 84     & 81     \\
ZO-Sign-SGD          & 80 & 89   & 78     & 80     \\
ZO-Adam              & 82 & 89   & 79     & 81     \\
Forward-Grad         & 87 & 89   & 78     & 83    \\
\midrule
\multicolumn{5}{c}{\texttt{OPT-13B}, WinoGrande}
\\
\midrule
FO-SGD               & 69.2 & 66.9 & 63.6   & 65.7   \\
FO-Adam              & 65.8 & 68.9 & 67.7   & 66.5   \\
\midrule
ZO-SGD               & 62.3 & 62.6 & 58.8   & 63.4   \\
ZO-SGD-MMT           & 60.9 & 64.0 & 58.6   & 63.8   \\
ZO-SGD-CONS          & 62.5 & 63.3 & 59.0   & 62.5   \\
ZO-Sign-SGD          & 62.1 & 63.4 & 59.0   & 63.8   \\
ZO-Adam              & 63.3 & 64.0 & 58.7   & 62.7   \\
Forward-Grad         & 64.4 & 62.9 & 59.4   & 61.8  \\
\midrule
\bottomrule[1pt]
\end{tabular}%
}
\end{table}


